Particle-based, rapid incremental smoother meets particle Gibbs

The particle-based, rapid incremental smoother (PARIS) is a sequential Monte Carlo technique allowing for efficient online approximation of expectations of additive functionals under Feynman--Kac path distributions. Under weak assumptions, the algorithm has linear computational complexity and limited memory requirements. It also comes with a number of non-asymptotic bounds and convergence results. However, being based on self-normalised importance sampling, the PARIS estimator is biased; its bias is inversely proportional to the number of particles but has been found to grow linearly with the time horizon under appropriate mixing conditions. In this work, we propose the Parisian particle Gibbs (PPG) sampler, whose complexity is essentially the same as that of the PARIS and which significantly reduces the bias for a given computational complexity at the price of a modest increase in the variance. This method is a wrapper in the sense that it uses the PARIS algorithm in the inner loop of particle Gibbs to form a bias-reduced version of the targeted quantities. We substantiate the PPG algorithm with theoretical results, including new bounds on bias and variance as well as deviation inequalities. We illustrate our theoretical results with numerical experiments supporting our claims.

==> introduction_backup.tex <==
This article addresses the problem of state estimation in general state-space hidden Markov models (HMMs) using sequential Monte Carlo (SMC) methods (also known as particle filters) and presents a novel online algorithm for computing smoothed expectations of additive state functions in models of this type.

Given a sequence of measurable spaces $\{(\xsp{n},\xfd{n}) \}_{n \in \nset}$ and $\{(\zsp{n},\zfd{n})\}_{n \in \nset}$, an HMM is a bivariate stochastic process $\{(X_n,Z_n)\}_{n \in \nset}$ where $(X_n,Z_n)$ takes value in $(\xsp{n} \times \zsp{n}, \xfd{n} \otimes \zfd{n})$, where  $\{X_n\}_{n \in \nset}$ (the state sequence) is a Markov chain that is only partially observed by the observation process $\{Z_n\}_{n \in \nset}$. Conditional to  the unobserved state sequence, the observations are assumed to be independent and the conditional distribution of each $Z_n$ depends only on the corresponding state $X_n$. HMMs are used today in a variety of scientific and engineering disciplines; see \cite{andrieu:doucet:2002,cappe:moulines:ryden:2005,chopin2020introduction}. Inference in HMMs typically involves computing conditional distributions of unobserved states given observations. Of particular interest are the sequences of filtering distributions, i.e., the conditional distributions of $X_{n}$ given $\chunk{Z}{0}{n}:=\left(Z_{0}, \ldots, Z_{n}\right)$ (our generic notation for vectors), and smoothing distributions, i.e., the joint conditional distributions of $\chunk{X}{0}{t}$ at $\chunk{Z}{0}{n}$, for $n \in \nset$. We  denote these distributions by $\phi_{n}$ and $\phi_{0: n \mid n}$.
In this paper, we focus on the problem of recursively computing smoothed expectations
\[
\phi_{0: n \mid n} h_{n}=\int h_{n}(\chunk{x}{0}{n}) \phi_{0: n \mid n}(\rmd \chunk{x}{0}{n}) \,, \quad n \in \nset \,.
\]
for additive functionals $h_{n}$ of form
$$
h_{n}(\chunk{x}{0}{n}):=\sum_{\ell=0}^{n-1} \tilde{h}_{\ell}(\chunk{x}{\ell}{\ell+1}) \quad\left( \chunk{x}{0}{n} \in \xpsp{0}{n}= \xsp{0} \times \cdots \times \xsp{n} \right)
$$
Expectations of this form appear for parameter estimation with the maximum likelihood method, for example in the calculation of the score function (the gradient of the log likelihood function) via the Fisher identity or in the calculation of the EM surrogate; see \cite{cappe:2001,andrieu:doucet:2003,poyiadjis:doucet:singh:2005,cappe:2009,poyiadjis:doucet:singh:2011}.
A particle filter approximates the flow $\left\{\phi_{n}\right\}_{n \in \nset}$ of filter distributions by a sequence of occupation measures associated with a swarm of particles $\{\epart{n}{i}\}_{i=1}^{N}$, $n \in \nset$. Particle filters revolve around two operations: a selection step duplicating/discarding particles with large/small importance weights, respectively, and a mutation step evolving randomly the selected particles in the state space. The most basic implementation is the bootstrap filter which propagates, in the mutation step, the particles according to the dynamics of the hidden Markov chain and selects the same multinomially according to importance weights proportional to the local likelihood of each particle given the current observation. This scheme imposes a dynamics of the particle cloud that resembles closely that of the filter distribution flow. Due to its very strong potential to solve non-linear filtering problems, SMC methods have been subject to extensive research during the last three decades, resulting in a broad range of developments and variations of the original scheme.


A limited Monte Carlo experiment is provided to illustrate our findings.

